Stability of Linear Structural Equation Models of Causal Inference

We consider the numerical stability of the parameter recovery problem in Linear Structural Equation Model ($\LSEM$) of causal inference. A long line of work starting from Wright (1920) has focused on understanding which sub-classes of $\LSEM$ allow for efficient parameter recovery. Despite decades of study, this question is not yet fully resolved. The goal of this paper is complementary to this line of work; we want to understand the stability of the recovery problem in the cases when efficient recovery is possible. Numerical stability of Pearl's notion of causality was first studied in Schulman and Srivastava (2016) using the concept of condition number where they provide ill-conditioned examples. In this work, we provide a condition number analysis for the $\LSEM$. First we prove that under a sufficient condition, for a certain sub-class of $\LSEM$ that are \emph{bow-free} (Brito and Pearl (2002)), the parameter recovery is stable. We further prove that \emph{randomly} chosen input parameters for this family satisfy the condition with a substantial probability. Hence for this family, on a large subset of parameter space, recovery is numerically stable. Next we construct an example of $\LSEM$ on four vertices with \emph{unbounded} condition number. We then corroborate our theoretical findings via simulations as well as real-world experiments for a sociology application. Finally, we provide a general heuristic for estimating the condition number of any $\LSEM$ instance.

==> Conclusion.tex <==
\section{Conclusion and Future Directions}
		In this paper, we initiate the study of condition number analysis for $\LSEM$s. We build theory and experiments to analyze the condition number for a class of instances. Further we give a heuristic that can be used in practice to identify if a given instance is \emph{well-conditioned}. This work opens a number of future directions. An immediate direction is to extend our understanding to other instances. In particular, can we prove condition number for \emph{every} bow-free graph? More generally, a series of recent works has extended the identifiability criteria beyond \emph{bow-free} graphs. Can we analyze the condition number of these larger class of instances? The other direction is to compute the condition number algorithmically. This can be approached by either trying to prove the correctness of the heuristic proposed in this paper, or coming up with a new algorithm. What happens for causal models
		other than LSEMs? In particular, are the ill-conditioned instances rare in a well-defined sense for Pearl's semi-Markovian causal model? 
		
		Finally, our results in this paper can be
		summarized as suggesting that while arbitrarily ill-conditioned instances exist they are rare and unlikely to arise in practice.
		Moreover, one may check how well-conditioned the instance at hand is. However, this statement depends on the underlying probability distribution on the instances. While our probability distribution is natural, it is desirable to achieve a more ``robust'' result. Smoothed analysis \cite{spielman2004smoothed} seems to be well-suited for this purpose. In particular, one could begin with smoothed analysis of ill-conditioned instances identified in the present paper.  
